Robust Classification Under $\ell_0$ Attack for the Gaussian Mixture Model

It is well-known that machine learning models are vulnerable to small but cleverly-designed adversarial perturbations that can cause misclassification. While there has been major progress in designing attacks and defenses for various adversarial settings, many fundamental and theoretical problems are yet to be resolved. In this paper, we consider classification in the presence of $\ell_0$-bounded adversarial perturbations, a.k.a. sparse attacks. This setting is significantly different from other $\ell_p$-adversarial settings, with $p\geq 1$, as the $\ell_0$-ball is non-convex and highly non-smooth. Under the assumption that data is distributed according to the Gaussian mixture model, our goal is to characterize the optimal robust classifier and the corresponding robust classification error as well as a variety of trade-offs between robustness, accuracy, and the adversary's budget. To this end, we develop a novel classification algorithm called FilTrun that has two main modules: Filtration and Truncation. The key idea of our method is to first filter out the non-robust coordinates of the input and then apply a carefully-designed truncated inner product for classification. By analyzing the performance of FilTrun, we derive an upper bound on the optimal robust classification error. We also find a lower bound by designing a specific adversarial strategy that enables us to derive the corresponding robust classifier and its achieved error. For the case that the covariance matrix of the Gaussian mixtures is diagonal, we show that as the input's dimension gets large, the upper and lower bounds converge; i.e. we characterize the asymptotically-optimal robust classifier. Throughout, we discuss several examples that illustrate interesting behaviors such as the existence of a phase transition for adversary's budget determining whether the effect of adversarial perturbation can be fully neutralized.

==> oldmaterial.tex <==
\section{Binary Symmetric mixture-Gaussian {\color{red} To be removed after reorganization}}
\label{sec:Gaussian-binary-symmetric}

%Let $Y \in \{-1,1\}$ be the true class variable such that $\pr{Y = 1} = \pr{Y =
%  -1} = 1/2$. Also, conditioned on $Y$, we assume that $\vX \sim \mN(Y \vmu,
%\Sigma)$ has a Gaussian distribution with mean $Y \vmu$ and covariance matrix
%$\Sigma$, where $\vmu \in \reals^d$ and $\Sigma$ is positive definite.
%An adversarial strategy with $l_0$ budget $k$ is a possibly randomized mapping
%from $Y, \vX$  to $\vXp \in \reals^d$ such that $\snorm{\vX - \vXp}_0 \leq k$,
%i.e.\ the adversary can modify at most $k$ coordinates in $\vX$ to obtain
%$\vXp$, so that the modified vector $\vXp$ is given to the classifier.
%{\color{red}[is it standard to assume that the adversary knows $Y$? I mean for
%  converse there is no harm in making adversary stronger, but I don't want to
%  write non-standard assumptions to make people confused.]} 
%A classifier is a function $\mC: \reals^d \rightarrow \{-1,1\}$. The loss
%associated to this classifier when there is an adversary with $l_0$ power $k$ is
%defined to be
%\begin{equation}
%  \label{eq:general-l0-loss-def}
%  \loss_{\vmu, \Sigma}(\mC, k) := \evwrt{\vX,Y}{\one{\ell^{(k)}(\mC; \vX, %Y)}},
%\end{equation}
%where
%\begin{equation*}
%  \ell^{(k)}(\mC; \vX, Y) := \one{\exists \vxp: \snorm{\vxp- \vX}_0 \leq k, \mC(\vxp) \neq Y}.
%\end{equation*}
%The optimal loss is defined by minimizing this over all possible classifiers:
%\begin{equation}
%  \label{eq:general-opt-loss-def}
%  \optloss_{\vmu, \Sigma}(k):= \inf_{\mC} %\loss_{\vmu, \Sigma}(\mC, k).
%\end{equation}

\subsection{Optimal Bayes classifier in the absence of adversary}
\label{sec:binary-symmeric-optimal-bayes-no-adv}


When $k=0$, or equivalently when the adversary is not present, it is easy to see
that the optimal Bayes classifier is the following MAP rule:
\begin{equation}
  \label{eq:binary-symmetric-no-adv-opt-bayes-rule}
  \mC_\text{Bayes}(\vXp) = \mC_\text{Bayes}(\vX) =
  \begin{cases}
    1 & \langle  \vw,  \vX  \rangle > 0 \\
    -1 & \text{otherwise},
  \end{cases}
\end{equation}
where
\begin{equation*}
  \vw = \Sigma^{-1} \vmu.
\end{equation*}
And using the symmetry, the corresponding misclassification error is
\begin{equation*}
  \optloss_{\vmu, \Sigma}(0) = \pr{\langle \vw, \vX \rangle \leq 0 | Y = 1} = \bar{\Phi}(\snorm{\vnu}_2),
\end{equation*}
where
\begin{equation*}
  \vnu := \Sigma^{-1/2} \vmu,
\end{equation*}
and
\begin{equation*}
  \bar{\Phi}(x) := \int_x^\infty \frac{1}{\sqrt{2\pi}} \exp(-t^2 / 2) dt.
\end{equation*}
Motivated by this, in order to have a meaningful asymptotic scenario as $d
\rightarrow \infty$, we may assume that
\begin{equation}
  \label{eq:binary-symmeric-norm-nu-1}
  \snorm{\vnu}_2 = 1.
\end{equation}




\subsection{A robuset classifier}
\label{sec:binary-symmetry-robust-classifier}

In this section, we introduce a classifier which we will show is robust against
adversarial attacks with $l_0$ power $k$. The classifier we propose is
parameterized by a subset $F \subset [d]$ which we will optimize for later. Given a
subset $F \subset [d]$, we introduce the classifier $\mC_F$ as follows
\begin{equation}
  \label{eq:robust-mC-F-def}
  \mC_F^{(k)}(\vXp) :=
  \begin{cases}
    1 & \langle  \vw(F^c), \vXp_{F^c} \rangle_k > 0\\
    -1 & \text{otherwise}
  \end{cases}
\end{equation}
where
\begin{equation*}
  \vw(F^c) := \Sigma_{F^c}^{-1} \vmu_{F^c},
\end{equation*}
and $\Sigma_{F^c}$ is the covariance matrix of $\vX_{F^c}$. 
{\color{red}[to add: a short discussion: compare with optimal Bayes and the
  highlight existence of truncation, $F$ is the set of coordinate we ``forget'',
  and it will be shown later that it will be important in some cases to indeed
  forget some coordinates.]}

\begin{prop}
\label{prop:upper-bound-ach}
  We have
  \begin{equation*}
    \loss_{\vmu, \Sigma}(\mC_F^{(k)}, k) \leq \frac{1}{\sqrt{2 \log d }} +\bar{\Phi}\left( \snorm{\vnu(F^c)}_2 - \frac{16 k \sqrt{\log d} \snorm{\tSigma_{F^c}^{1/2} \Sigma_{F^c}^{-1/2}}_\infty \snorm{\vnu(F^c)}_\infty}{\snorm{\vnu(F^c)}_2} \right),
  \end{equation*}
  where
  \begin{equation*}
    \vnu(F^c) := \Sigma_{F^c}^{-1/2} \vmu_{F^c}.
  \end{equation*}
\end{prop}

\begin{proof}
  Note that given $\vx \in \reals^d$, we have
  \begin{equation*}
    \ell^{(k)}(\mC_F^{(k)}; \vx, 1) = \one{\exists \vxp: \snorm{\vxp - \vx}_0 \leq k, \mC_F^{(k)}(\vxp) \neq 1} = \one{\exists \vxp \in \reals^d: \snorm{\vxp - \vx}_0 \leq k, \langle  \vw(F^c), \vxp_{F^c} \rangle \leq 0}
  \end{equation*}
  Using Lemma ??, for $\vxp$ such that $\snorm{\vxp - \vx}_0 \leq 0$, since
  $\snorm{\vxp_{F^c} - \vx_{F^c}}_0 \leq \snorm{\vxp - \vx}_0 \leq k$, we have
  \begin{equation*}
    |\langle  \vw(F^c), \vxp_{F^c} \rangle_k - \langle \vw(F^c), \vx_{F^c} \rangle| \leq 8k \snorm{\vw(F^c) \odot \vx_{F^c}}_\infty.
  \end{equation*}
  This means that
  \begin{equation*}
    \one{\exists \vxp \in \reals^d: \snorm{\vxp - \vx}_0 \leq k, \langle  \vw(F^c), \vxp_{F^c} \rangle \leq 0} \leq \one{\langle \vw(F^c) , \vx_{F^c} \rangle \leq 8k \snorm{\vw(F^c)\odot \vx_{F^c}}_\infty},
  \end{equation*}
  and
  \begin{equation}
\label{eq:ev-ellk-1-bound-1}
    \ev{\ell^{(k)}(\mC_F^{(k)}; \vX, 1) | Y=1} \leq \pr{\langle \vw(F^c), \vX_{F^c}  \rangle \leq 8k \snorm{\vw(F^c)\odot \vX_{F^c}}_\infty | Y= 1}.
  \end{equation}
  Let $\Sigma_{F^c}$ be the covariance matrix of the random vector $\vX_{F^c}$
  and let $\tSigma_{F^c}$ be the diagonal part of $\Sigma_{F^c}$. Since
  $\tSigma_{F^c}$ is diagonal, we may write
  \begin{equation}
    \label{eq:snorm-w-Fc-X-Fc-infty-bound-1}
    \snorm{\vw(F^c) \odot \vX_{F^c}}_\infty = \snorm{(\tSigma^{1/2} \vw(F^c)) \odot (\tSigma^{-1/2} \vX_{F^c})}_\infty \leq \snorm{\tSigma_{F^c}^{1/2} \vw(F^c)}_\infty \snorm{\tSigma_{F^c}^{-1/2} \vX_{F^c}}_\infty
  \end{equation}
Note that conditioned on $Y = 1$, for $i \in F^c$, the distribution of
coordinate $i$ in the random vector $\tSigma_{F^c}^{-1/2} \vX_{F^c}$ is
$\mN(\nu_i(F^c), 1)$. Hence, a simple union bound implies that
\begin{equation*}
  \pr{\snorm{\tSigma_{F^c}^{-1/2} \vX_{F^c}}_\infty > \snorm{\vnu(F^c)}_\infty + \sqrt{2 \log d}|Y=1} \leq \frac{1}{\sqrt{2 \log d}}.
\end{equation*}
Note that $\bar{Phi}(\snorm{\vnu(F^c)}_2)$ is the optimal Bayes
misclassification error of $Y$ given $\vX_{F^c}$, which is indeed not smaller
than the optimal Bayes misclassification error of $Y$ given $X$, which is in
turn equal to $\bar{\Phi}(\snorm{\vnu}_2)$. This means that $\snorm{\vnu(F^c)}_2
\leq \snorm{\vnu}_2 = 1$.  Consequently, we have $\snorm{\vnu(F^c)}_\infty
\leq \snorm{\vnu4(F^c)}_2 \leq 1$. Thereby, we get
\begin{equation}
\label{eq:pr-snorm-tSigma-X-logd-1}
  \pr{\snorm{\tSigma_{F^c}^{-1/2} \vX_{F^c}}_\infty > 2 \sqrt{\log d}|Y=1} \leq \frac{1}{\sqrt{2 \log d}}.
\end{equation}
On the other hand, we have
\begin{equation}
\label{eq:snorm-tsigma-w-bound-2}
  \snorm{\tSigma_{F^c}^{1/2} \vw(F^c)}_\infty = \snorm{\tSigma^{1/2}_{F^c} \Sigma_{F^c}^{-1/2} \vnu(F^c)}_\infty \leq \snorm{\tSigma^{1/2}_{F^c} \Sigma_{F^c}^{-1/2}}_\infty \snorm{\vnu(F^c)}_\infty.
\end{equation}
Using~\eqref{eq:snorm-w-Fc-X-Fc-infty-bound-1},
\eqref{eq:pr-snorm-tSigma-X-logd-1}, and~\eqref{eq:snorm-tsigma-w-bound-2} back
into~\eqref{eq:ev-ellk-1-bound-1} and simplifying, we get
\begin{align*}
  \ev{\ell^{(k)}(\mC_F^{(k)}; X, 1) | Y= 1} &\leq \frac{1}{\sqrt{2\log d}} + \pr{\langle \vw(F^c), \vX_{F^c}  \rangle \leq 16 k \sqrt{\log d}  \snorm{\tSigma^{1/2}_{F^c} \Sigma_{F^c}^{-1/2}}_\infty \snorm{\vnu(F^c)}_\infty | Y = 1} \\
  &= \frac{1}{\sqrt{2 \log d }} + \bar{\Phi}\left( \snorm{\vnu_{F^c}}_2 - \frac{16 k \sqrt{\log d} \snorm{\tSigma_{F^c}^{1/2} \Sigma_{F^c}^{-1/2}}_\infty \snorm{\vnu(F^c)}_\infty}{\snorm{\vnu(F^c)}_2} \right).
\end{align*}
% see expanded calculations on the ordinary note of 2021-01-11, maybe we need to
% expand it a little bit?
Due to the symmetry, we have the same bound conditioned on $Y=-1$ which yields
the desired result. 
\end{proof}



\subsection{An strategy for the Adversary with independence assumption}
\label{sec:binary-symmetric-adv-strategy-neutralize-set}

In this section, we assume that $\Sigma$ is diagonal, i.e.\ $X_i$'s are
independent conditioned on  $Y$, and denote the diagonal elements of $\Sigma$ by
$\sigma_1^2, \dots, \sigma_d^2$ where $\sigma_i^2 = \text{Var}(X_i)$.
A randomized strategy for the adversary with budget $k$ is defied to be a
distribution $P_{\vXp | \vX, Y}$ such that with probability one we have
$\snorm{\vXp - \vX}_0 \leq k$. We restrict ourselves to the set of strategies
such that $Y, \vX, \vXp$ have a joint density $f_{Y, \vX, \vXp}$ and denote
$\mA(k)$ to be the set of such random adversarial strategies with budget $k$.

\begin{lem}
\label{lem:error-lower-bound-adv-strategy}
For any random adversarial strategy $P_{\vXp|\vX, Y} \in \mA(k)$ with budget
$k$, we have
\begin{equation*}
  \optloss_{\vmu,\Sigma}(k) \geq \frac{1}{2} \pr{f_{\vXp|Y}(\vXp |1) = f_{\vXp|Y}(\vXp|-1)} + \pr{f_{\vXp|Y}(\vXp|-1) > f_{\vXp|Y}(\vXp|1) \bigg| Y = 1},
\end{equation*}
\end{lem}

\begin{proof}
  This is the Bayes optimal error associated with the MAP estimator, simplified
  using the symmetry assumption. {\color{red}[to expand?]}
\end{proof}

Now, we introduce a family of randomized strategies for the adversary,  parameterized
by  subsets $A \subset [d]$. Given $A \subset [d]$, having observed $Y$ and
$\vX$, the adversary follows the procedure explained below. For $i \in A$, if
$\sgn(X_i) = \sgn(Y\mu_i)$ {\color{red}[define $\sgn$ earlier in the document]}, then we define the random variable $I_i$ as
\begin{equation*}
  I_i :=
  \begin{cases}
    1 & \text{with probability  } 1 - p_i(X_i, Y) \\
    0 & \text{otherwise}
  \end{cases}
\end{equation*}
where
\begin{equation*}
  p_i(X_i, Y) := \frac{\exp(-(X_i + Y\mu_i)^2 / 2\sigma_i^2)}{\exp(-(X_i - Y\mu_i)^2 / 2\sigma_i^2)}.
\end{equation*}
Note that the condition $\sgn(X_i) = \sgn(Y\mu_i)$ ensures that $p_i(X_i, Y) \in
[0,1]$.
Otherwise, if $\sgn(X_i) \neq \sgn(Y \mu_i)$, we define $I_i = 0$. Next, we
define a random vector $\vZ \in \reals^d$ as follows. For $i \neq A$, let $Z_i
= X_i$. For $i \in A$, let $Z_i = X_i$ if  $I_i = 0$, and $Z_i = \xi_i$ where
$(\xi_i: i \in A)$ are i.i.d.\ random variables uniformly distributed in
$[-1/2,1/2]$ which are independent from everything else. It is easy to see that
\begin{equation}
  \label{eq:adv-Z-cond-f}
  f_{\vZ_A|Y}(\vec{z} | 1) = f_{\vZ_A|Y}(\vec{z} | -1) = \prod_{i \in A} \left[  \frac{1}{\sqrt{2 \pi \sigma_i^2}} \exp\left( - \frac{(|z_i| + |\mu_i|)^2}{2\sigma_i^2}\right) + \alpha_i \one{z_i \in [-1/2,1/2]}   \right],
\end{equation}
where for $i \in A$
\begin{equation*}
  \alpha_i = \pr{I_i = 1 | Y = 1} = \pr{I_i = 1| Y = -1} = \int_0^\infty [1-p_i(t,1)] f_{X_i|Y}(t|1) dt.
\end{equation*}
Finally, we define
$\vXp$ as follows:
\begin{equation}
  \label{eq:vXp-def-A}
  \vXp :=
  \begin{cases}
    \vZ & \text{if } \sum_{i \in A} I_i \leq  \snorm{\vnu_A}_1 \log d\\
    \vX & \text{o.t.w.}
  \end{cases}
\end{equation}
From this definition, it is evident that with probability one we have
\begin{equation}
  \label{eq:vXp-vX-norm-0-log-d-nu-A-1}
  \snorm{\vX - \vXp}_0 \leq \snorm{\vnu_A}_1 \log d,
\end{equation}
and hence the above introduces a randomized adversarial strategy in
$\mA(\snorm{\vnu_A}_1 \log d)$. 
We denote this randomized strategy for the adversary by $\adv(A)$. 
Now we use this together with
Lemma~\ref{lem:error-lower-bound-adv-strategy} to show the following result:

\begin{prop}
\label{prop:ind-low-bound-conv}
  For any subset $A \subset [d]$, we have
  \begin{equation*}
    \optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d) \geq \bar{\Phi}(\snorm{\vnu_{A^c}}_2) - \frac{1}{\log d}.
  \end{equation*}
\end{prop}

\begin{proof}
Note that when $A$ is empty, there is no adversarial modification and we the
standard Bayes analysis implies that 
$\optloss_{\vmu, \Sigma}(0) = \bar{\Phi}(\snorm{\vnu}_2) =
\bar{\Phi}(\snorm{\vnu_{A^c}}_2)$ and the desired bound holds. Hence, we may
assume that $A$ is nonempty for the rest of the proof.

  As we discussed above, due to~\eqref{eq:vXp-vX-norm-0-log-d-nu-A-1}, the 
  randomized strategy $\adv(A)$ for the adversary is in  $\mA(\snorm{\vnu}_1 \log d)$
  and we may use Lemma~\ref{lem:error-lower-bound-adv-strategy} to bound
  $\optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d)$ from below. Before that, we
  show that with high probability under the above randomized strategy for the
  adversary, we have $\sum_{i \in A} I_i \leq \snorm{\vnu_A}_1 \log d$ and hence
  $\vXp = \vZ$. It is easy to see that for each $i$, $\pr{I_i = 1| Y = 1} =
  \pr{I_i = 1 | Y = -1}$, therefore
  \begin{align*}
    \pr{I_i = 1} = \pr{I_i = 1 | Y = \sgn(\mu_i)} &= \int_{0}^\infty [1 - p_i(t, \sgn(\mu_i))] f_{X_i | Y}(t|\sgn(\mu_i)) d t \\
                                                  &= \int_0^\infty \left[ 1 - \frac{\exp(-(t+|\mu_i|)^2 / 2\sigma_i^2)}{\exp(-(t-|\mu_i|)^2 / 2\sigma_i^2)} \right]\exp\left( -(t-|\mu_i|)^2/2\sigma_i^2 \right) d t \\
                                                  &= 1 - e \bar{\Phi}(|\nu_i|) \\
                                                  &= \text{Erf}(|\nu_i|/\sqrt{2}) \\
    &\leq \left( \sqrt{\frac{2}{\pi}} |\nu_i|\right) \wedge 1
  \end{align*}
  Hence, we have
  \begin{equation*}
    \pr{I_i = 1} = \pr{I_1 = 1 | Y = 1} = \pr{I_i = 1 | Y = -1} \leq \left( \sqrt{\frac{2}{\pi}} |\nu_i|\right) \wedge 1.
  \end{equation*}
  Therefore, using Markov's inequality, if $I$ is the indicator of $\sum_{i \in
    A} I_i > \snorm{\vnu_A}_1 \log d$, we have
  \begin{equation}
    \label{eq:pr-I-1-bound-1-logd}
    \pr{I = 1 } = \pr{I= 1 | Y=1} = \pr{I = 1 | Y = -1}\leq \frac{\sqrt{2 / \pi} \sum_{i \in A} |\nu_i|}{\snorm{\vnu_A}_1 \log d} \leq \frac{1}{\log d}.
  \end{equation}
Now, we bound
  $\optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d)$ from below
 We do this in
  the following two cases. 


  \underline{Case 1: $A = [d]$}. In this case, using
  Lemma~\ref{lem:error-lower-bound-adv-strategy}, we have
  \begin{align*}
    \optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d ) &\geq \frac{1}{2} \pr{f_{\vXp | Y}(\vXp | 1) = f_{\vXp|Y}(\vXp | -1)} \\
                                                      &\stackrel{(a)}{=} \frac{1}{2} \pr{f_{\vXp | Y}(\vXp | 1) = f_{\vXp|Y}(\vXp | -1) | Y=1 } \\
                                                      &\geq \frac{1}{2} \pr{f_{\vXp | Y}(\vXp | 1) = f_{\vXp|Y}(\vXp | -1), I = 0 | Y = 1} \\
                                                      &\stackrel{(b)}{=} \frac{1}{2} \pr{f_{\vZ|Y}(\vZ | 1) = f_{\vZ|Y}(\vZ|-1) | Y = -1} \\
                                                      &\geq \frac{1}{2} \pr{f_{\vZ|Y}(\vZ | 1) = f_{\vZ|Y}(\vZ|-1) | Y = 1} - \frac{1}{2} \pr{I = 1|Y = 1}\\
                                                      &\stackrel{(c)}{\geq} \frac{1}{2} - \frac{1}{2 \log d}
  \end{align*}
  where $(a)$ uses the symmetry, $(b)$ uses the fact that when $I = 0$, by
  definition we have $\vXp = \vZ$, and $(c)$ uses~\eqref{eq:adv-Z-cond-f} and~\eqref{eq:pr-I-1-bound-1-logd}.

  \underline{Case 2: $A \subsetneqq [d]$}. Using
  Lemma~\ref{lem:error-lower-bound-adv-strategy}, we have
  \begin{equation}
    \label{eq:adv-lowerb-bound-use-lemma-case-2}
\begin{aligned}
    \optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d) &\geq \pr{f_{\vXp| Y}(\vXp | -1) > f_{\vXp|Y}(\vXp | 1) | Y=1} \\
    &\geq \pr{f_{\vXp| Y}(\vXp | -1) > f_{\vXp|Y}(\vXp | 1), I = 0 | Y=1} \\
    &\stackrel{(a)}{=}\pr{f_{\vZ| Y}(\vZ | -1) > f_{\vZ|Y}(\vZ | 1), I = 0 | Y=1} \\
    &\geq \pr{f_{\vZ| Y}(\vZ | -1) > f_{\vZ|Y}(\vZ | 1)| Y=1} - \pr{I = 1|Y = 1} \\
    &\stackrel{(b)}{\geq}  \pr{f_{\vZ| Y}(\vZ | -1) > f_{\vZ|Y}(\vZ | 1)| Y=1} - \frac{1}{\log d}
\end{aligned}
\end{equation}
where $(a)$ uses the fact that by definition, when $I=0$, we have $\vXp = \vZ$,
and $(b)$ uses~\eqref{eq:pr-I-1-bound-1-logd}.
Note that since $Z_i$ are conditionally independent given $Y$, we have
\begin{equation*}
  f_{\vZ|Y}(\vZ|Y) = f_{\vZ_A | Y} (\vZ_A|Y) f_{\vZ_{A^c}|Y}(\vZ_{A^c}|Y).
\end{equation*}
But from~\eqref{eq:adv-Z-cond-f}, we have $f_{\vZ_A|Y}(\vZ_A|1) =
f_{\vZ_A|Y}(\vZ_A|-1)$ a.s.. Using this
in~\eqref{eq:adv-lowerb-bound-use-lemma-case-2}, we get
\begin{equation*}
  \optloss_{\vmu, \Sigma}(\snorm{\vnu_A}_1 \log d) \geq \pr{f_{\vZ_{A^c}|Y}(\vZ_{A^c}|-1) > f_{\vZ_{A^c}|Y}(\vZ_{A^c}|1) | Y = 1} -\frac{1}{\log d} = \bar{\Phi}(\snorm{\vnu_{A^c}}_2) - \frac{1}{\log d}.
\end{equation*}

We may combine the two cases following the convention that when $A = [d]$, $A^c
= \emptyset$ and $\snorm{\vnu_{A^c}}_2 = 0$. This completes the proof.
\end{proof}

\subsection{Matching bounds for the independent case}
\label{sec:independent-matching-bounds}

In this section, under the condition that the covariance matrix $\Sigma$ is
diagonal, we simplify the bound in Proposition~\ref{prop:upper-bound-ach} and
show that it almost matches the bound in
Proposition~\ref{prop:ind-low-bound-conv} up to logarithmic terms.

Note that without loss of generality, we may assume that the coordinates are
ordered in a way that
\begin{equation*}
  |\nu_1| \geq |\nu_2| \geq \dots \geq |\nu_d|. 
\end{equation*}
Given $c \in (0,1)$, we define
\begin{equation}
  \label{eq:lambda-c-def}
  \lambda_c := \min \{t: \snorm{\vnu_{[1:t]}}_2 \geq c\}.
\end{equation}

{\color{red}[In the following theorem, the first bound works for $c \in [0,1)$
  while the second works for $c \in (0,1]$, will need to add this.]}

\begin{thm}
%  \label{thm:ind-bound-finite}
  If $\Sigma$ is diagonal and the coordinates in $\vnu$ are sorted, for $c \in
  (0,1)$, we have
  \begin{equation*}
    \optloss_{\vmu, \Sigma}\left( \frac{\snorm{\vnu_{[1:\lambda_c]}}_1}{\log d} \right) \leq \frac{1}{\sqrt{2 \log d}} + \bar{\Phi}\left( \sqrt{1-c^2} - \frac{16}{\sqrt{1-c^2} \sqrt{\log d}} \right ),    
  \end{equation*}
  and
  \begin{equation*}
  \optloss_{\vmu, \Sigma}(\snorm{\vnu_{[1:\lambda_c]}}_1 \log d) \geq \bar{\Phi}(\sqrt{1-c^2}) - \frac{1}{\log d}.    
  \end{equation*}
\end{thm}

\begin{rem}
Roughly speaking, Theorem~\ref{thm:ind-bound-finite} says that up to logarithmic
terms, we have
\begin{equation*}
  \optloss_{\vmu, \Sigma}(\snorm{\vnu_{[1:\lambda_c]}}_1) \approx \bar{\Phi}(\sqrt{1-c^2}).
\end{equation*}
\end{rem}

\begin{proof}[Proof of Theorem~\ref{thm:ind-bound-finite}]
 We use the bound in Proposition~\ref{prop:upper-bound-ach} with $F =
[1:\lambda_c-1]$. Since $\Sigma$ is diagonal, it is easy to see that
we have $\tSigma_{F^c} = \Sigma_{F^c}$, $\vw(F^c) = \vw_{F^c}$, and $\vnu(F^c) =
\vnu_{F^c}$. Therefore,  the bound in Proposition~\ref{prop:upper-bound-ach} with $k =
\snorm{\vnu_{[1:\lambda_c]}}_1 / \log d$ simplifies 
into the following
\begin{equation}
  \label{eq:ind-thm-ach-bound-simple}
  \optloss_{\vmu, \Sigma}\left( \frac{\snorm{\vnu_{[1:\lambda_c]}}_1}{\log d} \right) \leq \frac{1}{\sqrt{2 \log d}} + \bar{\Phi}\left( \snorm{\vnu_{[\lambda_c:d]}}_2 - \frac{\snorm{\vnu_{[1:\lambda_c]}}_1 \snorm{\vnu_{[\lambda_c: d]}}_\infty}{\snorm{\vnu_{[\lambda_c  : d]}}_2} \frac{16}{\sqrt{\log d}}\right).
\end{equation}
Note that we have
\begin{equation}
\label{eq;norm-2-vnu-lambda-c-d-bound}
  \snorm{\vnu_{[\lambda_c:d]}}_2^2  = 1- \snorm{\vnu_{1:\lambda_c-1}}_2^2 \geq 1 - c^2.
\end{equation}
% We have
% \begin{equation}
%   \label{eq:norm-2-vnu-lambdac+1:d-bound}
%   \begin{aligned}
%     \snorm{\vnu_{[\lambda_c+1:d]}}_2^2 &= 1 - \snorm{\vnu_{[1:\lambda_c]}}_2^2 \\
%     &\geq 1 - \frac{\lambda_c}{\lambda_c - 1} \snorm{\vnu_{[1:\lambda_c - 1]}}_2^2 \\
%     &\geq 1 - 2 \snorm{\vnu_{[1:\lambda_c-1]}}_2^2 \\
%     &\geq 1 - 2c^2.
%   \end{aligned}
% \end{equation}
On the other hand,
\begin{equation} 
  \label{eq:bound-lamnbda-c-norm-1-inf-bound}
  \begin{aligned}
    \snorm{\vnu_{[1:\lambda_c]}}_1 \snorm{\vnu_{[\lambda_c: d]}}_\infty & = \snorm{\vnu_{[1:\lambda_c]}}_1 |\nu_{\lambda_c}| \\
    &\leq \snorm{\vnu_{[1:\lambda_c]}}_2^2 \\
    &\leq \snorm{\vnu}_2^2 \\
    &= 1
  \end{aligned}
\end{equation}
Substituting~\eqref{eq;norm-2-vnu-lambda-c-d-bound}
and~\eqref{eq:bound-lamnbda-c-norm-1-inf-bound} back
into~\eqref{eq:ind-thm-ach-bound-simple}, we get
\begin{equation}
  \label{eq:ind-ach-bound-final-simple}
    \optloss_{\vmu, \Sigma}\left( \frac{\snorm{\vnu_{[1:\lambda_c]}}_1}{\log d} \right) \leq \frac{1}{\sqrt{2 \log d}} + \bar{\Phi}\left( \sqrt{1-c^2} - \frac{16}{\sqrt{1-c^2} \sqrt{\log d}} \right )
\end{equation}
Furthermore, with $A =[1:\lambda_c]$, the bound in
Proposition~\ref{prop:ind-low-bound-conv} implies that
\begin{equation}
  \label{eq:ind-conv-bound-simple}
  \optloss_{\vmu, \Sigma}(\snorm{\vnu_{[1:\lambda_c]}}_1 \log d) \geq \bar{\Phi}(\sqrt{1-c^2}) - \frac{1}{\log d}.
\end{equation}
This completes the proof.
\end{proof}

\subsection{Asymptotic Results in the independet case}
\label{sec:independent-asymp}

In this section, we study the asymptotic regime in the setup of
Section~\ref{sec:independent-matching-bounds} assuming that we have a sequence
$(\vmud, \Sigmad)$ where for each $d$, $\vmud \in \reals^{d}$ and
$\Sigmad$ is a diagonal covariance matrix with nonzero diagonal entries. We
define
\begin{equation*}
  \vnud := (\Sigmad)^{-1/2} \vmud.
\end{equation*}
Recalling from ??, in order to have a meaningful asymptotic regime
{\color{red}[improve wording and add reference]}, we may assume that 
\begin{equation}
\label{eq:vnud-norm-2-1}
  \snorm{\vnud}_2 = 1 \qquad \forall d.
\end{equation}
Furthermore, without loss of generality, we assume that with $\vnud = (\nud_1,
\dots, \nud_d)$, we have 
\begin{equation}
\label{eq:vnud-sorted}
  |\nud_1| \geq |\nud_2| \geq |\nud_d| \qquad \forall d.
\end{equation}
For each $d$  we define
\begin{equation}
  \label{eq:lambda-d-c-def}
  \lambdad_c := \min\{t: \snorm{\vnud_{[1:t]}}_2 \geq c\} \qquad \text{for } 0 < c \leq 1.
\end{equation}
Furthermore, for $0 < c \leq 1$, we define
\begin{equation}
  \label{eq:asymp-func-Psi-d-def}
  \funcd(c) := \log_d \snorm{\vnud_{[1:\lambdad_c]}}_1.
\end{equation}
Note that since $c  > 0$, $\lambdad_c \geq 1$ and
$\snorm{\vnud_{[1:\lambdad_c]}}_1 > 0$. Therefore, $\funcd(c)$  is well defined. 

It is easy to verify the following properties for the function $\funcd(.)$:

\begin{lem}
  \label{lem:funcd-props}
  $\funcd(.)$ is nonincreasing and $\funcd(c) \in [-1/2,1/2]$ for all $c \in
  (0,1]$. 
\end{lem}

\begin{proof}
  Note that
  \begin{equation*}
    \funcd(c) = \log_d \snorm{\vnud_{[1:\lambdad_c]}}_1 \leq \log_d \snorm{\vnud}_1 \leq \log_d (\sqrt{d} \snorm{\vnud}_2) = \log_d \sqrt{d} = \frac{1}{2}.
  \end{equation*}
  On the other hand, note that for $c > 0$, we have $\lambdad_c \geq 1$ and
  $\funcd(c) \geq \log_d |\nud_1| = \log_d \snorm{\vnu}_\infty$. Furthermore, we
  have $    1 = \snorm{\vnud}_2^2 \leq d \snorm{\vnud}_\infty$ which implies
  that $\snorm{\vnud}_\infty \geq 1/ \sqrt{d}$. Consequently, $\funcd(c) \geq
  \log_d 1/\sqrt{d} = -1/2$. This completes the proof.
\end{proof}

{\color{red}[motivate asymptotic analysis where we have a sequence of
  adversarial power $k_d$, and we essentially characterize the asymptotic
  behavior when $k_d \approx d^r$, and this characterization is based on $r$.  Also say
  that $\optloss_d$ is a shorthand for $\optloss_{\vmud, \Sigmad}$]}

{\color{red}we also need to emphasize early in the document that our strategy is
to ask the question  ``if we want the misclassification error to be at most
a value, then what is the maximum adversary power''. We can then do some
inversion to answer the main question ``given a certain adversarial power, what
is the minimum misclassification error''. In the context of this section, this
inversion can literally be done by taking the pseudo inverse of the function
$\funcinf$. I might add a corollary to Theorem~\ref{thm:asymp-independent} below
to address this inversion. This can perhaps be useful later when discussing examples.}

\begin{thm}
  \label{thm:asymp-independent}
  Assume that for all $c \in (0,1]$, $\funcd(c)$ converges to $\funcinf(c)$,
  i.e.\  $\funcd(.)$ converges pointwise to $\funcinf(.)$. Then $\funcinf(.)$
  is nondecreasing and with $\funcinf(0) := \lim_{c \downarrow 0} \funcinf(c)$,
  the following hold for all $c \in [0,1]$:
  \begin{enumerate}
  \item If $\limsup_{d \rightarrow \infty} \log_d k_d < \funcinf(c)$, then
    $\limsup_{d \rightarrow \infty} \optloss_d(k_d) \leq
    \bar{\Phi}(\sqrt{1-c^2})$.
  \item If If $\liminf_{d \rightarrow \infty} \log_d k_d > \funcinf(c)$, then
    $\liminf_{d \rightarrow \infty} \optloss_d(k_d) \geq 
    \bar{\Phi}(\sqrt{1-c^2})$.
  \end{enumerate}
\end{thm}

\begin{lem}
  \label{lem:func-inf-nonnegative}
  If $\funcinf(.)$  exists as in the above theorem, then $\funcinf(c) \in [0,1/2]$
  for all $c \in [0,1]$. 
\end{lem}

\begin{proof}
  For all $c>0$ and all $d$, we have
  \begin{equation*}
    \snorm{\vnud_{[1:\lambdad_c]}}_1 \geq \snorm{\vnud_{[1:\lambdad_c]}}_2^2 \geq c^2.
  \end{equation*}
  Therefore
  \begin{equation*}
    \funcinf(c) = \lim_{d \rightarrow \infty} \funcd(c) = \lim_{d \rightarrow \infty} \log_d \snorm{\vnud_{[1:\lambdad_c]}}_1 \geq \liminf_{d \rightarrow \infty} 2 \log_d c = 0.
  \end{equation*}
  Sending $c$ to zero we also realize that $\funcinf(0) \geq 0$.
\end{proof}

{\color{red}[the fact that $\funcinf(c) \in [0,1/2]$ has an important
  interpretation, especially if we discuss the pseudo inverse of $\funcinf$:
$1/2$ corresponds to adversarial power $\sqrt{d}$ and zero corresponds to
constant adversarial power.]}

\begin{proof}[Proof of Theorem~\ref{thm:asymp-independent}]
  Note that since $\funcd(.)$ is nondecreasing for all $d$, if $\funcinf(c) =
  \lim \funcd(c)$  exists, $\funcinf(.)$ is indeed nondecreasing and
  $\funcinf(0)$ is well defined.
  
\underline{Part 1} First we assume that $c \in (0,1)$. Since $\funcinf(c) = \lim
\funcd(c)$ and $\log \log d / \log d \rightarrow 0$, $\limsup \log_d k_d <
\funcinf(c)$ implies that for $d$ large enough, we have
\begin{equation*}
  \log_d k_d < \funcd(c) - \frac{\log \log d}{\log d}.
\end{equation*}
Thereby
\begin{equation*}
  \log_d k_d < \log_d \snorm{\vnud_{[1:\lambdad_c]}}_1 - \frac{\log \log d}{\log d} = \log_d \frac{ \snorm{\vnud_{[1:\lambdad_c]}}_1}{\log d}.
\end{equation*}
Hence, Theorem~\ref{thm:ind-bound-finite} implies that
\begin{equation*}
  \optloss_d(k_d) \leq \optloss_d\left( \frac{ \snorm{\vnud_{[1:\lambdad_c]}}_1}{\log d} \right) \leq \frac{1}{\sqrt{2 \log d}} + \bar{\Phi}\left( \sqrt{1-c^2} - \frac{16}{\sqrt{1-c^2} \sqrt{\log d}} \right).
\end{equation*}
Sending $d$ to infinity, we get $\limsup \optloss_d(k_d) \leq
\bar{\Phi}(\sqrt{1-c^2})$. Next, we consider $c =0$. Note that since
$\funcinf(.)$ is nondecreasing, $\limsup \log_d k_d < \funcinf(0)$ implies that
$\limsup \log_d k_d < \funcinf(c)$ for all $c > 0$. Consequently, the above
bound implies that $\limsup \optloss(k_d) \leq \bar{\Phi}(\sqrt{1-c^2 })$ for all
$c > 0$. Sending $c$ to zero, we realize that $\limsup \optloss(k_d) \leq
\bar{\Phi}(0)$. Finally, for $c = 1$, note that the classifier that always
outputs $1$ has misclassification error at most $1/2$. This implies that
irrespective of the sequence $k_d$, we always have $\limsup \optloss_d(k_d) \leq
1/2 = \bar{\Phi}(\sqrt{1-1^2})$ and the bound automatically holds for $c = 1$.

\underline{Part 2} First we assume that $c \in (0,1]$. Similar to the first
pare, $\liminf \log_d k_d > \funcinf(c)$ implies that for $d$ large enough, we
have
\begin{equation*}
  \log_d k_d > \funcd(c) + \frac{\log \log d}{\log d},
\end{equation*}
and
\begin{equation*}
    \log_d k_d > \log_d \snorm{\vnud_{[1:\lambdad_c]}}_1 + \frac{\log \log d}{\log d} = \log_d  (\log d\snorm{\vnud_{[1:\lambdad_c]}}_1).
  \end{equation*}
  Hence, Theorem~\ref{thm:ind-bound-finite} implies that
  \begin{equation*}
    \optloss_d(k_d) \geq \optloss_d(\log d \snorm{\vnud_{[1:\lambdad_c]}}_1) \geq \bar{\Phi}(\sqrt{1-c^2}) - \frac{1}{\log d}. 
  \end{equation*}
  Sending $d \rightarrow \infty$, we get $\liminf \optloss_d(k_d) \geq
  \bar{\Phi}(\sqrt{1-c^2})$. For the case $c = 0$, note that irrespective of the
  sequence $k_d$, we always have $\optloss_d(k_d) \geq \optloss_d(0) =
  \bar{\Phi}(\sqrt{1-0^2})$. Thereby, the result for $c =0$ automatically holds. 
\end{proof}


{\color{red} the inverse result, to motivate asking the inverse question}

For $\alpha \in [0,1]$, we define
\begin{equation}
  \label{eq:funcinf-inv-def}
  \funcinfinv(\alpha) := \inf \{ \bar{\Phi}(\sqrt{1-c^2}): \funcinf(c) \geq \alpha\} \wedge \frac{1}{2}.
\end{equation}

{\color{red} motivate the role of $1/2$: we can always get error 1/2 trivially,
  and if $\alpha > 1/2$, we always get $1/2$, since  $\funcinf(c) \leq 1/2$. I
  wanted this to be defined for $\alpha > 1/2$ as well, since $\log_d k_d \in
  [0,1]$.}

\begin{thm}
  \label{thm:ind-asymp-inv}
  In the setup of Theorem~\ref{thm:asymp-independent}, we have
  \begin{enumerate}
  \item If $\limsup \log_d k_d < \alpha$ then $\limsup \optloss_d(k_d) \leq
    \funcinfinv(\alpha)$.
  \item If $\liminf \log_d k_d > \alpha$ then $\liminf \optloss_d(k_d) \geq \funcinfinv(\alpha)$.
  \end{enumerate}
\end{thm}

\begin{proof}
  {\color{red} to be added.}
\end{proof}

\subsection{Discussion}
\label{sec:ind-discussion}

\begin{example}
  Let $\nud_i = 1/\sqrt{d}$ for $1 \leq i \leq d$, then
  \begin{center}
    \includegraphics[width=0.9\textwidth]{./temp/2021-01-14_1}
  \end{center}
\end{example}

\begin{example}
  Let
  \begin{equation*}
    \vnud = \left( \frac{\sqrt{1/\log d}}{1}, \frac{\sqrt{1/\log d}}{\sqrt{2}}, \frac{\sqrt{1/\log d}}{\sqrt{2}}, \dots,  \frac{\sqrt{1/\log d}}{\sqrt{d/2}}, \dots, \frac{\sqrt{1/ \log d}}{\sqrt{d/2}}\right)
  \end{equation*}
  {\color{red} to explain in words: we split the unit power in $\log d$
    blocks of exponential size growth: first block of size 1, second of size 2,
    third of size $4$ and the final of size $d/2$, and the power is uniformly
    distributed within each block.}

  $\funcinf(c) = c/2$ and
\begin{equation*}
    \funcinfinv(\alpha) =
    \begin{cases}
      \bar{\Phi}(\sqrt{1-(2\alpha)^2}) & 0 \leq \alpha \leq 1/2 \\
      \frac{1}{2} & 1/2 < \alpha \leq 1.
    \end{cases}
  \end{equation*}
    \begin{center}
    \includegraphics[width=0.9\textwidth]{./temp/2021-01-14_2}
  \end{center}

\end{example}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Note_01_Truncated_Mean"
%%% End:

